SAiD: Speech-driven Blendshape Facial Animation with Diffusion

Speech-driven 3D facial animation is challenging due to the scarcity of large-scale visual-audio datasets despite extensive research. Most prior works, typically focused on learning regression models on a small dataset using the method of least squares, encounter difficulties generating diverse lip movements from speech and require substantial effort in refining the generated outputs. To address these issues, we propose a speech-driven 3D facial animation with a diffusion model (SAiD), a lightweight Transformer-based U-Net with a cross-modality alignment bias between audio and visual to enhance lip synchronization. Moreover, we introduce BlendVOCA, a benchmark dataset of pairs of speech audio and parameters of a blendshape facial model, to address the scarcity of public resources. Our experimental results demonstrate that the proposed approach achieves comparable or superior performance in lip synchronization to baselines, ensures more diverse lip movements, and streamlines the animation editing process.

==> docs/problem.tex <==
\section{Problem Statement}\label{sec:problem}

The main objective is to generate realistic and diverse blendshape coefficient sequences using speech audio instead of the direct generation of facial motions.
We postulate a supervised learning scenario, leveraging a conditional generative model to address this problem.
The dataset used for the learning consists of pairs of speech waveforms and their associated sequences of blendshape coefficients.

\begin{itemize}
    \item Main goal: generate blendshape coefficients sequences conditioned on speech audio
\end{itemize}

